DisTime: Distribution-based Time Representation for Video Large Language Models

Despite advances in general video understanding, Video Large Language Models (Video-LLMs) face challenges in precise temporal localization due to discrete time representations and limited temporally aware datasets. Existing methods for temporal expression either conflate time with text-based numerical values, add a series of dedicated temporal tokens, or regress time using specialized temporal grounding heads. To address these issues, we introduce DisTime, a lightweight framework designed to enhance temporal comprehension in Video-LLMs. DisTime employs a learnable token to create a continuous temporal embedding space and incorporates a Distribution-based Time Decoder that generates temporal probability distributions, effectively mitigating boundary ambiguities and maintaining temporal continuity. Additionally, the Distribution-based Time Encoder re-encodes timestamps to provide time markers for Video-LLMs. To overcome temporal granularity limitations in existing datasets, we propose an automated annotation paradigm that combines the captioning capabilities of Video-LLMs with the localization expertise of dedicated temporal models. This leads to the creation of InternVid-TG, a substantial dataset with 1.25M temporally grounded events across 179k videos, surpassing ActivityNet-Caption by 55 times. Extensive experiments demonstrate that DisTime achieves state-of-the-art performance across benchmarks in three time-sensitive tasks while maintaining competitive performance in Video QA tasks. Code and data are released at https://github.com/josephzpng/DisTime.

==> tables/ablation_ensemble.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering
\begin{tabular}{c|ll}

Method   & mIoU  & R1@50 \\ \hline

UniMD    & 26.63 & 22.22 \\

Mr.Blip  & 39.81 & 34.34 \\

TFVTG    & 38.95 & 40.40 \\
\rowcolor[HTML]{EFEFEF} 
Ensemble & \textbf{43.97} & \textbf{45.45}
\end{tabular}
\caption{xxx}
\label{tab:ensemble}
\end{table}

==> tables/ablation_frames.tex <==
\begin{table}[ht]
\vspace{-3mm}
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{c|cccc|ccc}
\hline
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{\textbf{Charades-STA (MR)}} & \multicolumn{3}{c}{\textbf{YouCook2 (DVC)}} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{$\text{\#frames}$}} & \begin{tabular}[c]{@{}c@{}}R@1\textsubscript{IoU=0.3} \end{tabular} & \begin{tabular}[c]{@{}c@{}}R@1\textsubscript{IoU=0.5}\end{tabular} & \begin{tabular}[c]{@{}c@{}}R@1\textsubscript{IoU=0.7}\end{tabular} & \begin{tabular}[c]{@{}c@{}}mIoU\end{tabular}& \begin{tabular}[c]{@{}c@{}}SODA\_c\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIDEr\end{tabular} & \begin{tabular}[c]{@{}c@{}}F1 Score\end{tabular} \\ \hline

\multicolumn{1}{c|}{8} &74.5 &49.2 &21.0 &46.9 &3.7 &14.1 &17.6 \\

\multicolumn{1}{c|}{16} &78.1 &\underline{56.3} &\textbf{29.7} &\textbf{51.6} &\textbf{4.2} &\textbf{15.6} &\textbf{20.5} \\

\multicolumn{1}{c|}{24} &\textbf{79.0} &\textbf{56.7} &\underline{28.8} &\textbf{51.6} &3.7 &13.2 &\underline{19.7}\\
 
\multicolumn{1}{c|}{32} &\underline{78.8} &56.0 &26.5 &\underline{50.5} &\underline{4.0} &\underline{15.1} & 19.2 \\
\hline
\end{tabular}
}
\vspace{-3.5mm}
\caption{Ablation study on the number of sampled frames.}
\label{tab:ablation_frames}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|cccc|ccc}
% \hline
%    & \multicolumn{4}{c|}{\textbf{Charades-STA}} & \multicolumn{3}{c}{\textbf{ActivityNet Captions}} \\ 
% \multirow{2}{*}{\textbf{\#decoder reg\underline{max}}} &
%   \begin{tabular}[c]{@{}c@{}}R@1\\ (IoU=0.3)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}R@1\\ (IoU=0.5)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}R@1\\ (IoU=0.7)\end{tabular} &
%   mIoU &
%   SODA\_c &
%   CIDEr &
%   METEOR \\ \hline
%    & 77.6      & 54.4     & 27.6     & 50.2     & 4.4            & 16.2            & 4.4            \\
% 32 & 77.4      & 54.8     & 27.7     & 50.5     & 4.5            & 18.9            & 4.9            \\
% 64 & 77.0      & 53.7     & 27.4     & 50.3     & 4.0            & 15.0            & 4.2            \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:dec_regmax}
% \end{table}

==> tables/ablation_latency.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}


\begin{table}[ht]
\vspace{-3mm}
\centering
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{c|c|cc}
\hline
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{2}{c}{\textbf{Latency (ms)} with 1*A100-80G}  \\ 
% \cline{3-4}
\multicolumn{1}{c|}{\multirow{-2}{*}{Method}} & \multicolumn{1}{c|}{\multirow{-2}{*}{Size}} & \begin{tabular}[c]{@{}c@{}} w/ Time Tokenizer \end{tabular} & \begin{tabular}[c]{@{}c@{}}w/o Time Tokenizer \end{tabular} \\ \hline

DisTime\textsubscript{InternVL} & 1B   & 420 ($\uparrow$2.94\%) & 408 \\

% DisTime\textsubscript{LLaVA-OV} & 7B   &- & - \\

DisTime\textsubscript{InternVL} & 8B   &722 ($\uparrow$2.70\%) & 703 \\

\hline
\end{tabular}
}
\vspace{-3.5mm}
\caption{Ablation study on the latency (ms) of time tokenizer.}
\label{tab:ablation_latency}
\end{table}

==> tables/ablation_predformat.tex <==
\begin{table}[ht]
\vspace{-3mm}
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{c|cccc|ccc}
\hline
\multicolumn{1}{c|}{} & \multicolumn{4}{c|}{\textbf{Charades-STA (MR)}} & \multicolumn{3}{c}{\textbf{YouCook2 (DVC)}} \\
\multicolumn{1}{c|}{\multirow{-2}{*}{$\text{\#}\text{method}$}} & \begin{tabular}[c]{@{}c@{}}R@1\textsubscript{IoU=0.3} \end{tabular} & \begin{tabular}[c]{@{}c@{}}R@1\textsubscript{IoU=0.5}\end{tabular} & \begin{tabular}[c]{@{}c@{}}R@1\textsubscript{IoU=0.7}\end{tabular} & \begin{tabular}[c]{@{}c@{}}mIoU\end{tabular}& \begin{tabular}[c]{@{}c@{}}SODA\_c\end{tabular} & \begin{tabular}[c]{@{}c@{}}CIDEr\end{tabular} & \begin{tabular}[c]{@{}c@{}}F1 Score\end{tabular} \\ \hline

\multicolumn{1}{c|}{Discrete} &33.4 &20.1 &8.7 &22.4 &0.5 &1.1 &2.5 \\

\multicolumn{1}{c|}{Text} &38.8 &26.4  &11.8 &26.3 &0.5 &1.0 &2.7\\

\multicolumn{1}{c|}{DisTime} &\textbf{78.1} &\textbf{56.3} &\textbf{29.7} &\textbf{51.6} &\textbf{4.2} &\textbf{15.6} &\textbf{20.5} \\

\hline
\end{tabular}
}
\vspace{-3.5mm}
\caption{
% Ablation study on methods for integrating timestamp tokens. ``Discrete'' uses multiple special tokens to represent timestamps, whereas ``Text'' processes timestamps into a text format.
Ablation study on time expression. ``Discrete'' uses multiple special tokens, whereas ``Text'' uses text-domain tokens.
}
\label{tab:ablation_predformat}
\end{table}

% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[t]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c|cccc|ccc}
% \hline
%    & \multicolumn{4}{c|}{\textbf{Charades-STA}} & \multicolumn{3}{c}{\textbf{ActivityNet Captions}} \\ 
% \multirow{2}{*}{\textbf{\#decoder reg\textsubscript{max}}} &
%   \begin{tabular}[c]{@{}c@{}}R@1\\ (IoU=0.3)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}R@1\\ (IoU=0.5)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}R@1\\ (IoU=0.7)\end{tabular} &
%   mIoU &
%   SODA\_c &
%   CIDEr &
%   METEOR \\ \hline
%    & 77.6      & 54.4     & 27.6     & 50.2     & 4.4            & 16.2            & 4.4            \\
% 32 & 77.4      & 54.8     & 27.7     & 50.5     & 4.5            & 18.9            & 4.9            \\
% 64 & 77.0      & 53.7     & 27.4     & 50.3     & 4.0            & 15.0            & 4.2            \\ \hline
% \end{tabular}%
% }
% \caption{}
% \label{tab:dec_regmax}
% \end{table}

==> tables/debug.tex <==
\begin{table}[!t]
\centering
\resizebox{.4\columnwidth}{!}{%
\begin{tabular}{c|c}
\hline
\textbf{Size} & \textbf{Model} \\ \hline
1B & InternVL2.5 \\
7B & LLaVA-OneVision \\
8B & InternVL2.5 \\
\hline
\end{tabular}
}
\vspace{-2mm}
\caption{
Details of the training data covering both general video understanding and time-sensitive comprehension.
}
\label{tab:training_data_dist}
\end{table}
